Decoding and Diversity in Machine Translation

Neural Machine Translation (NMT) systems are typically evaluated using automated metrics that assess the agreement between generated translations and ground truth candidates. To improve systems with respect to these metrics, NLP researchers employ a variety of heuristic techniques, including searching for the conditional mode (vs. sampling) and incorporating various training heuristics (e.g., label smoothing). While search strategies significantly improve BLEU score, they yield deterministic outputs that lack the diversity of human translations. Moreover, search tends to bias the distribution of translated gender pronouns. This makes human-level BLEU a misleading benchmark in that modern MT systems cannot approach human-level BLEU while simultaneously maintaining human-level translation diversity. In this paper, we characterize distributional differences between generated and real translations, examining the cost in diversity paid for the BLEU scores enjoyed by NMT. Moreover, our study implicates search as a salient source of known bias when translating gender pronouns.

==> sections/introduction_old.tex <==
% \section{Introduction}
% Neural machine translation (NMT) is an end-to-end learning approach for translation. 
% 
% 
Neural machine translation (NMT) is currently the dominant approach to machine translation (MT). 
NMT systems typically consist of a two stage pipeline:
(i) fitting a conditional language model (using neural networks) 
by optimizing a probabilistic objective;
then (ii) searching for the ``best translation'', e.g., via beam search. 
While step (i) consists of probabilistic modeling,
practitioners are typically focused on the step (ii) decodings,
not with how well they have modeled the distribution over possible translations.
Moreover, popular evaluation metrics, including BLEU \cite{papineni2002bleu}, 
ROUGE \cite{Lin2003ROUGERU}, and METEOR \cite{banerjee2005meteor},
which measure agreement with human-authored candidate translations,
provide only a very indirect incentive to match the (conditional) distribution of translations.
While these metrics are justified by reproducibility and their correlation 
with human perceptions of translation quality,
a singular focus on these metrics 
has led to a neglect of other important desiderata,
% including generating translations 
such as the degree to which translations 
\emph{reflect the diversity of real-world language}.
Diversity in NMT is valuable for numerous reasons:
(i) issues of societal representation, e.g., when translating
between a non-gendered and gendered language,
maximum likelihood decoders would always choose the most likely gender; %%%%%%%%% TODO 
(ii) homogeneity can make NMT outputs monotonous and less engaging to users;
(iii) individuals who interact with language primarily through NMT
might develop a warped exposure to that language.

% \gn{Is this actually a desideratum? It might be necessary to argue why reflecting the diversity of real-world language is actually necessary for translation, either through a citation or intuitive argument.}.
%%%%%%%%%%% TODO these? 
Notably, optimizing these metrics may even require
eliminating diversity. 
For example, if in a particular context 
the French word ``estranger'' would be translated 
to ``stranger'' 70\% of the time 
and to  ``outsider'' 30\% of the time,
the expected BLEU score is optimized by always choosing ``stranger'' 
% \gn{Only if this is done in a way that is insensitive to context. Many would argue that there very few words that are genuinely substitutable for each-other in every context (e.g. see \url{https://www.researchgate.net/profile/Ruediger_Schreyer/publication/243460514_Synonyms_in_Context/links/00b4951d4001ea979a000000.pdf}). 
% If prediction of these translations is done in a context-sensitive way then predicting as accurately as possible is the optimal strategy.}.

In this paper, we investigate the distributional dissimilarity 
between NMT outputs and natural translations.
We confirm the efficacy of deterministic decoding as quantified via BLEU,
% The gains due to beam search, which attempts to identify the mode of the conditional distribution, are pronounced.
showing that an NMT model trained for only $1/3$ of an epoch 
and decoded via beam search can match 
a fully trained model decoded by sampling from the softmax.
% \gn{``sampling'' coming here might be a little bit sudden for some readers, 
% who might think that the ``opposite'' of beam search is greedy search, 
% since it's so rare to generate from MT models using sampling. Maybe this contrast could be made earlier.}. 
% Presumably, if we had an infinitely expressive model and infinite amount of data, and an oracle optimizer, 
% sampling would with temperature 1 would give us 
Moreover, the fully trained model gains nearly 14 BLEU points 
when we decode deterministically via beam search versus by sampling.
%Thus, there exists a trade-off between diversity and BLEU. 
% \gn{Although you haven't presented any evidence that the sampling-based system generates more diverse outputs (and by what measure of diversity) in the intro yet.}.
%One way to explore this trade-off is 
%to tune the softmax temperature \cite{ACKLEY1985147}. 
Thus, there exists a trade-off between diversity and BLEU which can be negotiated by tuning the softmax temperature \cite{ACKLEY1985147}. 
% 
% 
Note that while NMT systems are sometimes rated 
against ``human-level'' performance 
(calculated via BLEU on sentences with multiple available translations \cite{ott2018analyzing}), %\cite{ott2018analyzing, DBLP:journals/corr/abs-1802-01886, shu-etal-2019-generating}),
this comparison is misleading.
NMT models are dialed to the extreme operating point
exhibiting zero diversity (conditional on input),
and then compared to human translations
that exhibit considerable diversity. % \cite{ott2018analyzing}. % \gn{What is the evidence for the statement that human translators demonstrate similar diversity as models sampled with temperature one? Do you have multiple references for the same sentence from human translators where you could assess this?}.

To examine this behavior, we propose a panel 
of diversity diagnostics for NMT systems.
% 
% This is important --- Nick, Davis, have you read this paper???
% 
%\gn{There are many methods for evaluating diversity in NLG systems, for example see the related works section of \citet{tevet2020evaluating} for a survey. How is the current work positioned in this area?}. 
These include distributional similarity comparisons of $n$-grams to the references (unlike distinct-ngrams \cite{li-etal-2016-diversity}), 
sentence length, punctuation, copy rates, 
and domain confusion scores using both linear discriminators with TF-IDF features
and BERT-based models used as discriminators \cite{devlin-etal-2019-bert} to distinguish between generated and real translations. %(unlike \citet{tevet2020evaluating}, who measure sentence similarity). 
%Our measure of distributional similarity of $n$-grams is done on the corpus level and is compared to the reference, which differs from distinct-ngrams \cite{li-etal-2016-diversity}. We 
Our study centers on the WMT 2017 German-English (De-En), 
English-German (En-De), and WMT 2014 French-English (Fr-En) datasets. % for achieving human-level translation quality:
Along the way, we make another related discovery:
that the singular focus on metrics like BLEU
can blind researchers to the consequences of 
ad hoc decisions that may improve BLEU 
while undermining probilistic interpretations of the learning objective. 
For example, \citet{ott2018analyzing}
investigated the distributions learned in stage (i) of NMT.
However a key finding of theirs---that NMT 
``smears probability mass in the hypothesis space''---turns 
out to be a foreseeable consequence
of label smoothing \cite{szegedy2016rethinking},
a popular heuristic that spreads mass across all labels 
(thus overweighting tokens) during training. 
% %%%%%%% TODO clarify this
% 
Interestingly, while this fact is not reported in the paper,
we confirmed it by inspecting their code. 

Finally, we ask whether the gains in performance due to search are \emph{worth it},
i.e., do gains in BLEU due to better decoding correspond to comparable gains 
in human judgments of quality as those due to better modeling. 
To this end, we conduct a human study and, to our surprise,
find that gains achieved via these two routes indeed do
correspond to similar gains in human assessments.
We make our code publicly available. %%%%%%%% TODO what code?

%provoke thought and promote discussion about diversity in NMT.


% \begin{itemize}
%     \itemsep0em 
%     \item An apples-to-apples comparison is strikingly less favorable for current NMT systems as compared to humans
%     \item Composing the outputs of a conditional language model with search heuristics produces outputs which are less diverse according to a variety of desiderata captured in our diagnostics
%     \item Sampling from the softmax tends to produce outputs which are more diverse (i.e. closer to human-level diversity) 
%     \item Label smoothing dramatically reduces diversity 
% \end{itemize}


%Lastly, we present a study involving human annotators in which we find that for a fixed BLEU score, sampling tends to produce more fluent output than beam search while maintaining similar adequacy. 
\input{tables/comparemt}

% D: (we should also figure out how graham's code is doing the above, or write our own script to analyze).
% D: simple caption: Rare unigrams like `She' and `her' are severely underpredicted when decoding with beam search. Decoding with sampling is able to retrieve 90% of feminine gender pronouns.
% N: original: $n$-gram occurrences according and \% match against the reference on the WMT17 De-En test set. Sampling is done on a model trained to convergence and beam search is done on a model trained for only $\frac{1}{3}$ of an epoch such that both methods achieve a BLEU score of 16 on the test set. A beam width of 10 was used for beam search. `her' was the third highest $n$-gram according to \% match where sampling outperformed beam search, and `She' was the ninth.



% TODO keep this?
%A more honest comparison of an NMT model to a human annotator should demonstrate performance subject to the constraint that the model also exhibit comparable diversity to that of the human annotator. An ideal NMT model would produce translations which simultaneously capture meaning adequately and fluently and produce translations which are similar in distribution to those of human annotators. We measure this similarity in distribution by considering a variety of desiderata includes similarity to the distributions of vocabulary, sentence length, and grammatical constructions of humans as well as distinguishability between human translations and those generated by the model. 


% Neural machine translation (NMT) is a sequence-to-sequence translation task that typically combines techniques like label smoothing \cite{szegedy2016rethinking}, heuristic decoding algorithms like beam search, and increasingly better architectures \cite{bahdanau2014neural,gehring2017convolutional,vaswani2017attention} in effort to improve translation quality. Translation quality is typically measured using automatic evaluation measures such as the bilingual evaluation understudy (BLEU) score \cite{papineni2002bleu}, the recall-oriented understudy for gisting evaluation (ROUGE) score \cite{Lin2003ROUGERU}, or the metric for evaluation of translation with explicit ordering (METEOR) score \cite{banerjee2005meteor}. Of these, BLEU is the most widely used %\todo{cite a bunch of papers using BLEU score}. 

% Each of these scores in some way measures concordance between the model output and a reference translation produced by a human, and each of them are correlated with human assessments. Using these measures of evaluation, human-level performance is typically measured by how well a translation produced by a human annotator agrees with the reference translation. %Furthermore, human-level diversity is often measures by pairwise BLEU \todo{Citation?}. 

% A variety of techniques are used to improve BLEU score, including beam search and label smoothing. However, outputs of a sequence-to-sequence model (in other words, a conditional language model) followed by a search strategy such as beam search produces deterministic outputs, and inherently exhibits no conditional entropy. Humans, on the other hand, exhibit a considerable amount of diversity in translations. In this way, we claim that the comparison of sequence-to-sequence NMT models evaluated using BLEU score is an apples-to-oranges comparison to humans, even if the NMT model achieves a `human-level' BLEU score. Furthermore, if the intention is to model the conditional distribution of translations, performing search would not be a coherent modeling choice in the first place. 

% A more honest comparison of an NMT model to a human annotator should demonstrate performance subject to the constraint that the model also exhibit comparable diversity to that of the human annotator. An ideal NMT model would produce translations which simultaneously capture meaning adequately and fluently and produce translations which are similar in distribution to those of human annotators. We measure this similarity in distribution by considering a variety of desiderata includes similarity to the distributions of vocabulary, sentence length, and grammatical constructions of humans as well as distinguishability between human translations and those generated by the model. 

% In this work, we demonstrate the following on the WMT 2014 German to English (en-de), English to German (de-en), and French to English (fr-en) datasets for achieving human-level translation quality:
% \begin{itemize}
%     \item Composing the outputs of a conditional language model with search heuristics produces outputs which are less diverse according to a variety of desiderata 
%     \item Sampling from the softmax (greedy decoding) tends to produce outputs which are more diverse (i.e. closer to human-level diversity) according to a variety of desiderata
%     \item An apples-to-apples comparison is strikingly less favorable for current NMT systems as compared to humans
% \end{itemize}

% %Lastly, we present a study involving human annotators in which we find that for a fixed BLEU score, sampling tends to produce more fluent output than beam search while maintaining similar adequacy. 

% We note in passing that the use of another popular strategy for improving BLEU score, label smoothing, is inherently at odds with the probabilistic modeling objective. We find that label smoothing coupled with beam search can improve BLEU score, but at the cost of dramatically reducing diversity measured by a variety of desiderata. 




% 
%  OLD BACKUP
% 

% The approach typically involves learning a probabilistic model as one part of a two stage pipeline. 
% Practitioners are often concerned with the best translation, not the distribution of translations. The second stage of this pipeline involves applying a search strategy (often beam search) to the resulting conditional distribution to estimate the most likely translation. Popular metrics of evaluation include the widely used BLEU score \todo{cite a bunch of papers using BLEU score} \cite{papineni2002bleu}, ROUGE score \cite{Lin2003ROUGERU}, and METEOR score \cite{banerjee2005meteor}. Each of these measures a degree of concordance with human evaluation by similarity of translations produced by the model to reference translations. Human-level performance is typically measured by comparing human output to references. 
% % Z: Be clear that this is even conditional on input
% %    A good way to make the point: give the same example to 2 different workers
% %       (or even the same worker on a different day!)
% %       and you'll get a different translation!
% Outputs of a sequence-to-sequence model 
% (in other words, a conditional language model) 
% followed by a search strategy such as beam search produces deterministic outputs conditional on the source sentence, 
% and exhibits no conditional entropy. 
% In contrast, two annotators can produce different translations of the same source sentence. 
% In this way, we claim that the comparison of sequence-to-sequence NMT models 
% evaluated using BLEU score is an apples-to-oranges comparison to humans, 
% even if the NMT model achieves a `human-level' BLEU score. 


% %-- probabilistic modeling etc, approached via a two stage pipeline, like clf tasks, typically concerned with best translation, not distribution - describe search first, what are metrics, precise methods ppl use to improve metrics. mention why these metrics are used in the first place - why theyre believed to have concordance w human eval --- 



% % Often times practitioners apply a search algorithm to the model output to estimate the most likely translation. 
% % search strategies during decoding


% %Neural machine translation (NMT) is a sequence-to-sequence translation task 
% %that typically combines techniques like label smoothing \cite{szegedy2016rethinking}, 
% %heuristic decoding algorithms like beam search, 
% %and increasingly better architectures \cite{bahdanau2014neural,gehring2017convolutional,vaswani2017attention}
% %in effort to improve translation quality.
% %Translation quality is typically measured using automatic evaluation measures 
% %such as the bilingual evaluation understudy (BLEU) score \cite{papineni2002bleu}, 
% %the recall-oriented understudy for gisting evaluation (ROUGE) score \cite{Lin2003ROUGERU},
% %or the metric for evaluation of translation with explicit ordering (METEOR) score \cite{banerjee2005meteor}. 
% %Of these, BLEU is the most widely used %\todo{cite a bunch of papers using BLEU score}. 

% %Each of these scores measures a notion of concordance 
% %between the model output and a reference translation produced by a human,
% %and each of them are correlated with human assessments. 
% %Using these measures of evaluation, human-level performance is typically measured 
% %by how well a translation produced by a human annotator agrees with the reference translation. %Furthermore, human-level diversity is often measures by pairwise BLEU \todo{Citation?}. 


% In this work, we propose a panel of novel diversity diagnostics for NMT systems, which captures phenomenon in both stages of the NMT pipeline (probabilistic modeling and search). These include distributional similarity comparisons of $n$-grams, sentence length, punctuation, copy rates, the ability to fool a linear discriminator with TF-IDF features, and the ability to fool a BERT-based discriminator. We demonstrate the following on the WMT 2017 German to English (En-De), English to German (De-En), and the WMT 2014 French to English (Fr-En) datasets:% for achieving human-level translation quality:
% \begin{itemize}
%     \itemsep0em 
%     \item An apples-to-apples comparison is strikingly less favorable for current NMT systems as compared to humans
%     \item Composing the outputs of a conditional language model with search heuristics produces outputs which are less diverse according to a variety of desiderata captured in our diagnostics
%     \item Sampling from the softmax tends to produce outputs which are more diverse (i.e. closer to human-level diversity) 
%     \item Label smoothing dramatically reduces diversity 
% \end{itemize}

% Finally, we make our code publicly available to promote the adoption of diversity diagnostics. 

% %Lastly, we present a study involving human annotators in which we find that for a fixed BLEU score, sampling tends to produce more fluent output than beam search while maintaining similar adequacy. 

% \begin{figure}
%   \centering
%   %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \includegraphics[width=0.5\textwidth]{figures/pairwise.pdf}
%   \caption{Trade-off between diversity and BLEU score compared to human-level performance in terms of BLEU and pairwise BLEU. For sampling, pairwise BLEU is measured over 10 samples. For beam search with a width of at least 2, pairwise BLEU is measured over the sequences in the beam.}
%   \label{fig:pairwise}
% \end{figure}

% % TODO keep this?
% %A more honest comparison of an NMT model to a human annotator should demonstrate performance subject to the constraint that the model also exhibit comparable diversity to that of the human annotator. An ideal NMT model would produce translations which simultaneously capture meaning adequately and fluently and produce translations which are similar in distribution to those of human annotators. We measure this similarity in distribution by considering a variety of desiderata includes similarity to the distributions of vocabulary, sentence length, and grammatical constructions of humans as well as distinguishability between human translations and those generated by the model. 


% % Neural machine translation (NMT) is a sequence-to-sequence translation task that typically combines techniques like label smoothing \cite{szegedy2016rethinking}, heuristic decoding algorithms like beam search, and increasingly better architectures \cite{bahdanau2014neural,gehring2017convolutional,vaswani2017attention} in effort to improve translation quality. Translation quality is typically measured using automatic evaluation measures such as the bilingual evaluation understudy (BLEU) score \cite{papineni2002bleu}, the recall-oriented understudy for gisting evaluation (ROUGE) score \cite{Lin2003ROUGERU}, or the metric for evaluation of translation with explicit ordering (METEOR) score \cite{banerjee2005meteor}. Of these, BLEU is the most widely used %\todo{cite a bunch of papers using BLEU score}. 

% % Each of these scores in some way measures concordance between the model output and a reference translation produced by a human, and each of them are correlated with human assessments. Using these measures of evaluation, human-level performance is typically measured by how well a translation produced by a human annotator agrees with the reference translation. %Furthermore, human-level diversity is often measures by pairwise BLEU \todo{Citation?}. 

% % A variety of techniques are used to improve BLEU score, including beam search and label smoothing. However, outputs of a sequence-to-sequence model (in other words, a conditional language model) followed by a search strategy such as beam search produces deterministic outputs, and inherently exhibits no conditional entropy. Humans, on the other hand, exhibit a considerable amount of diversity in translations. In this way, we claim that the comparison of sequence-to-sequence NMT models evaluated using BLEU score is an apples-to-oranges comparison to humans, even if the NMT model achieves a `human-level' BLEU score. Furthermore, if the intention is to model the conditional distribution of translations, performing search would not be a coherent modeling choice in the first place. 

% % A more honest comparison of an NMT model to a human annotator should demonstrate performance subject to the constraint that the model also exhibit comparable diversity to that of the human annotator. An ideal NMT model would produce translations which simultaneously capture meaning adequately and fluently and produce translations which are similar in distribution to those of human annotators. We measure this similarity in distribution by considering a variety of desiderata includes similarity to the distributions of vocabulary, sentence length, and grammatical constructions of humans as well as distinguishability between human translations and those generated by the model. 

% % In this work, we demonstrate the following on the WMT 2014 German to English (en-de), English to German (de-en), and French to English (fr-en) datasets for achieving human-level translation quality:
% % \begin{itemize}
% %     \item Composing the outputs of a conditional language model with search heuristics produces outputs which are less diverse according to a variety of desiderata 
% %     \item Sampling from the softmax (greedy decoding) tends to produce outputs which are more diverse (i.e. closer to human-level diversity) according to a variety of desiderata
% %     \item An apples-to-apples comparison is strikingly less favorable for current NMT systems as compared to humans
% % \end{itemize}

% % %Lastly, we present a study involving human annotators in which we find that for a fixed BLEU score, sampling tends to produce more fluent output than beam search while maintaining similar adequacy. 

% % We note in passing that the use of another popular strategy for improving BLEU score, label smoothing, is inherently at odds with the probabilistic modeling objective. We find that label smoothing coupled with beam search can improve BLEU score, but at the cost of dramatically reducing diversity measured by a variety of desiderata. 



==> tables/big_table.tex <==
\newcommand\rotation{30} % Amt to rotate top row text
\begin{table*}[ht]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize
	\addtolength{\tabcolsep}{-3.8pt}

\begin{tabu}{@{}ll@{\hskip 8pt}lllllllll@{\hskip 8pt}llllll@{}}
\multicolumn{1}{p{2.5ex}}{\rotatebox{0}{\textbf{Model (cased)}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=1.0}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.9}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.8}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.7}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.6}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.5}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.4}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.3}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.2}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Sampling T=0.1}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=1}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=2}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=4}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=6}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=8}}} &
\multicolumn{1}{p{2.5ex}}{\rotatebox{\rotation}{\textsc{Beam k=10}}} \\
\toprule 
Unigram L1 & 82.6 & \textbf{99.4} & 83.4 & 77.8 & 83.0 & 96.3 & 86.3 & 81.3 & 94.9 & 71.7 & 74.7 & \textbf{74.1} & 88.3 & -- & -- & -- \\
TFIDF Discr. L1 & 84.2* & 97.0 & 80.0 & \textbf{82.3}* & 79.6 & \textbf{97.6}* & 89.4* & 83.1* & 96.5* & 73.6* & 84.7* & 71.2 & \textbf{92.4}*   & 111.2 & 59.2  & 1.88 \\
Metric X & 84.8* & 97.2 & 80.7 & 82.0* & 82.7 & \textbf{97.6}* & 86.4 & 84.3* & 92.8 & 77.0* & 83.4* & 72.8 & 91.9*  & 128.1 & 63.6 & 2.02 \\
Metrix Y & 85.4* & 97.3 & 83.5 & 77.8 & 81.9 & 97.0 & \textbf{91.4}* & \textbf{90.1}* & 96.2* & 80.7* & 81.0* & 69.8 & 91.9*  &  213.5 &  87.9 & 2.42 \\
Metric Z & \textbf{86.5}* & 97.8 &\textbf{84.6}* & 79.1* & \textbf{84.1}* & 96.8 & 90.8* & 88.9* & \textbf{96.8}* & \textbf{83.4}* & \textbf{85.5}* & 70.2 & 91.4*    & 194.0 & 77.9 & 2.49 \\
BLEU & \textbf{86.5}* & 97.8 &\textbf{84.6}* & 79.1* & \textbf{84.1}* & 96.8 & 90.8* & 88.9* & \textbf{96.8}* & \textbf{83.4}* & \textbf{85.5}* & 70.2 & 91.4*    & 194.0 & 77.9 & 2.49 \\
\midrule
\textit{Something Else} & \textit{88.6} & \textit{97.5} & \textit{90.0} & \textit{87.3} & \textit{83.9} & \textit{92.2} & \textit{85.0} & \textit{86.9} & \textit{97.0} & \textit{84.9} & \textit{88.1} & \textit{86.6} & \textit{90.9} & -- & -- & -- \\
\bottomrule

\end{tabu}
\end{minipage}
\caption{Perhaps we should do diff from validation set. e.g. if unigram L1 for the model is 1.5 and unigram L1 for validation set (against test set) is 0.5, then the result is +1.0. Then we can make this a heat map. More negative more red, more positive more green, closer to zero more black.}
\label{table:accuracy-blimp}
\end{table*}

==> tables/she.tex <==
\begin{table}[ht]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize
\begin{tabu}{@{}lccc@{}}
\toprule
\textbf{Unigram} &  \textbf{Match}  & \textbf{Sampling} & \textbf{Beam} \\
\midrule
her & 0.9048 & 18 & 1 \\
She & 0.8889 & 7 & 0 \\
\bottomrule
\end{tabu}
\end{minipage}
\vspace{10px}
\caption{Unigrams like `She' and `her' are underrepresented in the outputs of beam search. According to a smoothed probability of unigrams being matched to the reference via sampling as opposed to beam search (described in \citet{DBLP:journals/corr/abs-1903-07926}), female gender pronouns are more likely to be produced by sampling.}
\label{table:female_table}

\todo{Just get rid of this table, since this is represented in figure 2.}

\vspace{10px}
\end{table}

\clearpage

==> tables/tradeoff.tex <==
\begin{figure}
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[width=0.5\textwidth]{figures/en_de/pairwise.pdf}
  \caption{Plotting BLEU against Pairwise BLEU (a measure of diversity) of the fully convolutional model from \cite{ott2018analyzing} trained on the WMT17 German English task. Pairwise BLEU is computed over 10 conditionally independent samples (sampling) and over the k sequences from width-k beams.}
  \label{fig:pairwise}
\end{figure}

==> tables/turkish.tex <==
\begin{table*}[h]
\section{Translation from a language without gendered pronouns to English}
\label{app:tren}
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize
\begin{tabu}{@{}lcccc@{}}
\toprule
System & Languages &  Original & Translation & Back translation \\
\midrule
\toprule

A 
& En-Tr-En    
& \begin{tabular}[x]{@{}c@{}} She took her girlfriend\\ to the movies. \end{tabular} 
& \begin{tabular}[x]{@{}c@{}} Kız arkadaşını \\ sinemaya götürdü.
 \end{tabular} 
& \begin{tabular}[x]{@{}c@{}} He brought his boyfriend \\ to the cinema.
\end{tabular} \\

B 
& En-Hi-En    
& \begin{tabular}[x]{@{}c@{}} She took her girlfriend\\ to the movies. \end{tabular} 
& \begin{tabular}[x]{@{}c@{}} वह अपनी प्रेमि का को फिल्मों में ले गया।

 \end{tabular} 
& \begin{tabular}[x]{@{}c@{}} He took his girlfriend \\ to the movies.
\end{tabular} \\
                
\bottomrule
\end{tabu}
\end{minipage}
\caption{TODO}
\label{table:turkish}
\end{table*}

